Complex contraction on trees without proof of correlation decay

We prove complex contraction for zero-free regions of counting weighted set cover problem in which an element can appear in an unbounded number of sets, thus obtaining fully polynomial-time approximation schemes(FPTAS) via Barvinok's algorithmic paradigm\cite{barvinok2016combinatorics}. Relying on the computation tree expansion, our approach does not need proof of correlation decay in the real axis. We directly look in the complex plane for a region that contracts into its interior as the tree recursion procedure goes from leaves to the root. For the class of problems under the framework of weighted set covers, we are able to give a general approach for describing the contraction regions and draw a unified algorithmic conclusion. Several previous results, including counting (weighted-)edge covers, counting bipartite independent sets and counting monotone CNFs can be completely or partially covered by our main theorem. In contrast to the correlation decay method which also depends on tree expansions and needs different potential functions for different problems, our approach is more generic in the sense that our contraction region for different problems shares a common shape in the complex plane.

==> anti-ferro.tex <==
\section{Anti-Ferromagnetic 2-spin Systems}
In this section, we provide a proof of complex contraction for anti-ferromagnetic 2-spin systems with bounded degree. 

Fix nonnegative $\beta, \gamma$ such that $\sqrt{\beta\gamma} \le \frac{\Delta - 2}{\Delta}$, $\beta > 0$. For $d \ge \frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}}$, define 
\begin{align}
    \tilde{x}(d) \triangleq \begin{cases}
        \frac{-1 - \beta\gamma + d(1 - \beta\gamma) - \sqrt{(-1 - \beta\gamma + d (1 - \beta\gamma))^2 - 4\beta\gamma}}{2 \gamma}, ~~~&\text{ for } \gamma > 0, \\
        \frac{\beta}{d - 1}, ~~~&\text{ for } \gamma = 0,
    \end{cases}
\end{align}
to be a root of the equation
\begin{align}\label{eq:anti-ferro:root}
    \frac{d(1-\beta\gamma) x}{(x + \beta)(\gamma x + 1)} = 1.
\end{align}
And denote 
\begin{align}
    \lambda_c(d) \triangleq \tilde{x}(d) \left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right)^d.
\end{align}

\begin{claim}\label{claim:anti-ferro:tilde-x-d}
    For $\beta\gamma < 1$ and $d \ge \frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}}$, we have $(-1 - \beta\gamma + d (1 - \beta\gamma))^2 - 4\beta\gamma \ge 0$. Further if $\gamma > 0$, there also holds $\tilde{x}(d) \le \sqrt{\frac{\beta}{\gamma}}$. 
\end{claim}
\begin{proof}
    Note that for $d \ge \frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}}$, we have 
    \begin{align}\label{eq:tilde-x-d}
    -1 - \beta\gamma + d (1 - \beta\gamma) \ge -1 - \beta\gamma + \frac{(1 + \sqrt{\beta\gamma})(1 - \beta\gamma)}{1 - \sqrt{\beta\gamma}} = -1 - \beta\gamma + (1 + \sqrt{\beta\gamma})^2 = 2\sqrt{\beta\gamma}.
    \end{align}
    
    Further, observe that
    \begin{align*}
        &\qquad\qquad \tilde{x}(d) \le \sqrt{\beta/\gamma}, \\
        &\iff -1 - \beta\gamma + d(1 - \beta\gamma) - \sqrt{(-1 - \beta\gamma + d (1 - \beta\gamma))^2 - 4\beta\gamma} \le 2\sqrt{\beta\gamma}, \\
        &\iff -1 - \beta\gamma + d(1 - \beta\gamma) - 2\sqrt{\beta\gamma} \le \sqrt{(-1 - \beta\gamma + d (1 - \beta\gamma))^2 - 4\beta\gamma}, \\
        &\iff 2\sqrt{\beta\gamma} \le -1 - \beta\gamma + d(1 - \beta\gamma),
    \end{align*}
    which has been proved in Equation (\ref{eq:tilde-x-d}).
\end{proof}

\begin{claim}
    For $\beta \le 1$, $\lambda_c(d)$ is strictly decreasing when $d \ge \frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}}$. 
    For $\beta > 1$, $\lambda_c(d)$ is strictly decreasing when $d \le d_0$ which $d_0$ 
\end{claim}
\begin{proof}
    Note that
    \begin{align*}
        \lambda_c'(d) &= \left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right)^d \left(\tilde{x}'(d) + \tilde{x}(d) \left(\ln\left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right) + \frac{d(1 - \beta\gamma)\tilde{x}'(d)}{(\beta + \tilde{x}(d))(1 + \gamma \tilde{x}(d))}\right)\right) \\
        &= \left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right)^d \left( 2 \tilde{x}'(d) + \tilde{x}(d) \ln\left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right) \right) \\
        &= \left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right)^d \left( -\frac{2 (1 - \beta\gamma) \tilde{x}(d)}{\sqrt{(-1-\beta\gamma + d(1 - \beta\gamma))^2 - 4 \beta\gamma}}  + \tilde{x}(d) \ln\left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right) \right).
    \end{align*}
    
    Now consider the function 
    \begin{align*}
        \Psi(d) =  -\frac{2 (1 - \beta\gamma)}{\sqrt{(-1-\beta\gamma + d(1 - \beta\gamma))^2 - 4 \beta\gamma}}  +  \ln\left(\frac{\tilde{x}(d) + \beta}{\gamma \tilde{x}(d) + 1}\right).
    \end{align*}
    With $\psi(x) = \frac{x + \beta}{\gamma x + 1} $ is an increasing function when $x \ge 0$ and $\tilde{x}(d)$ is decreasing with respect to $d$, we know that $\Psi(d)$ is a 
\end{proof}

And denote
\begin{align}
    \lambda_c \triangleq \min_{\frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}} \le d \le \Delta - 1} \lambda_c(d).
\end{align}


Recall that the recursion function for 2-spin systems is 
\begin{align*}
    f_{\lambda, d}(z_1, z_2, \cdots, z_d) \triangleq \lambda \prod_{i=1}^d \left(\frac{\gamma z_i + 1}{z_i + \beta}\right).
\end{align*}
Denote $\hat{x}(\lambda, d)$ is the unique fix point on $(0, +\infty)$ to the function $\hat{f}_{\lambda, d}(x) = \lambda \left(\frac{\gamma x + 1}{x + \beta}\right)^d$, i.e., 
\begin{align*}
    \hat{f}_{\lambda, d}(\hat{x}(\lambda, d)) = \hat{x}(\lambda, d).
\end{align*}


\begin{claim}
    For $\lambda < \lambda_c$, we have 
    \[|\hat{f}_{\lambda, d}'(\hat{x}(\lambda, d))| = \frac{d(1 - \beta\gamma) \hat{x}(\lambda, d)}{(\gamma \hat{x}(\lambda, d) + 1)(\hat{x}(\lambda, d) + \beta)} < 1,\]
    for all $d \in [\Delta - 1]$. 
\end{claim}
\begin{proof}
    We first prove that $\hat{x}(\lambda, d) < \tilde{x}(d)$ for $d \ge \frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}}$. Otherwise, based on the function $\hat{f}_{\lambda, d}$ is a decreasing function on $[0, +\infty)$, we have 
    \begin{align*}
        \hat{f}_{\lambda, d}(\tilde{x}(d)) \ge \hat{f}_{\lambda, d}(\hat{x}(\lambda, d)) = \hat{x}(\lambda, d) \ge \tilde{x}(d) = \lambda_c(d) \left( \frac{\gamma \tilde{x}(d) + 1}{\tilde{x}(d) + \beta} \right)^d > \hat{f}_{\lambda, d}(\tilde{x}(d)),
    \end{align*}
    which is a contradiction. 

    Denote \[\psi(x) = \frac{d (1 - \beta\gamma) x}{(\gamma x + 1)(x + \beta)}.\]
    
    For $\gamma = 0$, the function $\psi(x) = \frac{d x}{x + \beta}$ is strictly increasing on $[0, +\infty)$ and therefore
    \[
    \psi(\hat{x}(\lambda, d)) < \psi(\tilde{x}(d)) = \frac{d \tilde{x}(d)}{\tilde{x}(d) + \beta} = 1.
    \]
    
    On the other hand, for $\gamma > 0$, the function $\psi(x)$ is strictly increasing when $x < \sqrt{\beta/\gamma}$ and strictly decreasing when $x > \sqrt{\beta/\gamma}$.
    Consequently, for $d < \frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}}$, we have
    \begin{align*}
        \psi(\hat{x}(\lambda, d)) \le \psi(\sqrt{\beta/\gamma}) = \frac{d(1 - \beta\gamma)}{(1 + \sqrt{\beta\gamma})^2} = \frac{d(1 - \sqrt{\beta\gamma})}{1 + \sqrt{\beta\gamma}} < 1. 
    \end{align*}
    Moreover, for $d \ge \frac{1 + \sqrt{\beta\gamma}}{1 - \sqrt{\beta\gamma}}$, recalling that $\hat{x}(\lambda, d) < \tilde{x}(d) \le \sqrt{\beta/\gamma}$ (c.f. Claim \ref{claim:anti-ferro:tilde-x-d}), there holds
    \begin{align*}
        \psi(\hat{x}(\lambda, d)) < \psi(\tilde{x}(d)) = 1,
    \end{align*}
    where we have recalled that $\tilde{x}(d)$ is a root of the equation $\psi(x) = 1$ (c.f. Equation (\ref{eq:anti-ferro:root})).
\end{proof}



\begin{thm}\label{thm:anti-ferro}
    For $\lambda_0 < \lambda_c$, setting 
    \begin{align*}
        x_0 = \frac{2(1 -\beta\gamma)\hat{x}}{\beta - \gamma \hat{x}^2} + \ln\left(\frac{\gamma\hat{x} + 1}{\hat{x} + \beta}\right), ~~~ x_1 = 
    \end{align*}
    where $\hat{x} = \min_{d \in [\Delta-1]}\{\hat{x}_{\lambda_0, d}\}$
    there exists $k > 0$ and $\delta > 0$ such that for any $\lambda \in \gU([0, \lambda_0], \delta)$, 
    \begin{align*}
        \ln\left(\frac{}{}\right)
    \end{align*}
\end{thm}

We just need to prove following lemma.
\begin{lemma}
    Suppose that $\lambda_0$ satisfies the condition in Theorem \ref{thm:anti-ferro}. Then there exists $x_0, x_1, k, \delta$ such that 
    \begin{enumerate}
        \item $\{0, -\ln(\beta), \ln(\gamma)\} \subseteq U(x_0, x_1, k)$
    \end{enumerate}
\end{lemma}

==> ferro.tex <==
\section{Ferromagnetic 2-spin systems}
Let $A= \left[\begin{array}{ll}{A_{0,0}} & {A_{0,1}} \\ {A_{1,0}} & {A_{1,1}}\end{array}\right] = \left[\begin{array}{ll}{\beta} & {1} \\ {1} & {\gamma}\end{array}\right]$ and $b_0 = 1, b_1 = \lambda$. 
The partition function of 2-spin systems with the graph $G = (V, E)$ is given by
\begin{equation}
Z^{\beta, \gamma}_G(\lambda) = \sum_{\sigma \in \{0, 1\}^V} \prod_{(u, v) \in E} A_{\sigma(u), \sigma(v)} \prod_{v \in V} b_{\sigma(v)}
\end{equation}

In this section, we focus on ferromagnetic 2-spin systems, i.e., $\beta \gamma > 1$, with unbounded maximum degree. 
Based on the result in \cite{chen2020rapid}, we just need to consider the zeros of partition function of trees with pinned leaves.
\begin{thm}[{Theorem 11. in \cite{chen2020rapid}}]
    Let $G = (V, E)$ be a connected graph. There exists a tree $T_G$ with pinned leaves such that $Z^{\beta, \gamma}_{G}(\lambda)$ divides $Z^{\beta, \gamma}_{T_{G}}(\lambda)$ as a polynomial on $\lambda$.
\end{thm}
Define 
\begin{align*}
    R^{\beta, \gamma, \lambda}(G, v) \triangleq \frac{Z^{\beta, \gamma}_{\sigma(v)=1}(\lambda)}{Z^{\beta, \gamma}_{\sigma(v)=0}(\lambda)}.
\end{align*}
Given a tree $T$ rooted at $v$, and assume that $u_1, \dots, u_d$ are the neighbours of $v$ and $T_i$ are subtrees rooted at $u_i$ for $i \in [d]$. It can be shown that
\begin{align*}
    R^{\beta, \gamma, \lambda}(T, v) = f_{\lambda, d}(R^{\beta, \gamma, \lambda}(T_1, v_1), \dots, R^{\beta, \gamma, \lambda}(T_d, v_d)),
\end{align*}
where 
\begin{align*}
    f_{\lambda, d}(z_1, z_2, \cdots, z_d) \triangleq \lambda \prod_{i=1}^d \left(\frac{\gamma z_i + 1}{z_i + \beta}\right).
\end{align*}


Similar to hard-core models, we define complex contraction as follows.
\begin{definition}
    We say $\lambda \in \sC$ satisfies complex-contraction property for unbounded 2-spin systems with parameters $\beta, \gamma$ if there is an close domain $F_{\lambda} \subseteq \hat{\sC}$ such that 
    \begin{enumerate}
        \item $\{\lambda, 0, \infty\} \subseteq F_{\lambda}, -1 \notin F_{\lambda}$,
        \item $f_{\lambda, d}(z_1, \dots, z_{d}) \in F_{\lambda}$ for any $d \ge 1$ and $z_i \in F_{\lambda}, i = 1, \dots, d$.
    \end{enumerate}
\end{definition}
\begin{remark}
    Different from the definition of complex contraction for hard-core models, we need $\{\lambda, 0, \infty\} \subseteq F_{\lambda}$ for 2-spin systems by observing that
    \begin{align*}
        R^{\beta, \gamma, \lambda}(\{v\}, v) = \begin{cases}
            \lambda, ~~~&\text{ for free vertex } v, \\
            0, ~~~&\text{ for vertex $v$ pinned by $0$}, \\
            \infty, ~~~&\text{ for vertex $v$ pinned by $1$}.
        \end{cases}
    \end{align*}
\end{remark}

\begin{lemma}
    If $\lambda$ satisfies complex-contraction property for unbounded 2-spin systems, then $Z^{\beta, \gamma}_G(\lambda) \neq 0$ for any graph. 
\end{lemma}

\subsection{Complex Contraction}
In this section, we provide a proof of complex contraction for ferromagnetic unbounded 2-spin systems.
\begin{thm}
    Suppose that $\beta > \gamma, \beta\gamma > 1, \gamma \le 1$. Denote $\lambda_c = \left( \frac{\beta}{\gamma} \right)^{\frac{\sqrt{\beta\gamma}}{\sqrt{\beta\gamma} - 1}}$. 
    For $\lambda_0 \in [\sqrt{\frac{\beta}{\gamma}}, \lambda_c)$, there exists $\delta > 0$ such that for any $\lambda \in \gU([0, \lambda_0], \delta)$ complex-contraction property holds for $\lambda$.
\end{thm}
Similar to hard-core models, we need a potential function $\phi$ to allow us deal with sum of same regions. Setting $\phi(w) = \ln\left( \frac{\gamma w + 1}{w + \beta} \right)$, we have $\phi^{-1}(w) = \frac{\beta \exp(w) - 1}{\gamma - \exp(w)}$ and
\begin{align*}
    f^{\phi}_{\lambda, d}(w_1, \dots, w_d) &= \phi(f_{\lambda, d}(\phi^{-1}(w_1), \dots, \phi^{-1}(w_d))) \\
    &= \ln\left(\frac{\gamma \lambda \exp(\sum_{i=1}^d w_i) + 1}{\lambda \exp(\sum_{i=1}^d w_i) + \beta}\right).
\end{align*}

Our goal is to find a convex region $U_{\lambda}$ as follows. 
\begin{lemma}\label{lem:ferro:complex-contraction}
    For $\lambda \in \sC$, if there exists convex and close region $U_{\lambda} \subseteq \{z: |\im{z}| < \pi \}$ such that 
    \begin{enumerate}
        \item $\{0, -\ln(\beta), \ln(\gamma)\} \subseteq U_{\lambda}$, $-1 \notin \phi^{-1}(U_{\lambda})$,
        \item $g_{\lambda}( d U_{\lambda}) \subseteq U_{\lambda}$ where
        $
            g_{\lambda}(z) = \ln\left( \frac{\gamma \lambda e^{z} + 1}{\lambda e^{z} + \beta} \right),
        $ for any $d \ge 1$.
    \end{enumerate}
    then $\lambda$ satisfies complex-contraction property.
\end{lemma}

We choose following class isosceles triangles for finding  $U_{\lambda}$:
\begin{align}
    U(x_1, k) = \{z: \re(z) \in [-x_1, 0], |\im(z)| \le k |\re(z)|\},
\end{align}
with $x_1 > 0, k > 0$.
The reason we put the apex in the origin is that
\begin{align}\label{def:tilde-U}
    d U(x_1, k) \subseteq \tilde{U}(k) \triangleq \{z: \re(z) \le 0, |\im(z)| \le k |\re(z)|\}.
\end{align}

\begin{lemma}
    For $\beta > 1 \ge \gamma$, we have $\{0, -\ln(\beta), \ln(\gamma)\} \subseteq U(x_1, k)$. 
    And $-1 \notin \phi^{-1}(U(x_1, k))$ for $x_1 = \ln\left( \frac{\beta^2 - 1}{\beta - \gamma} \right)$.
\end{lemma}
\begin{proof}
    For $\gamma < 1$, we have $\phi(-1) = \ln\left(\frac{1 - \gamma}{\beta - 1}\right) < -\ln\left( \frac{\beta^2 - 1}{\beta - \gamma} \right)$, thus $-1 \notin h(W_k)$. \\
    For $\gamma = 1$, we have $-1 \notin \phi^{-1}(U(x_1, k))$ if and only if $0 \in \exp(U(x_1, k))$ which is impossible. 
\end{proof}


\begin{lemma}\label{lem:ferro:real}
    For $\beta > 1 \ge \gamma$ and $\lambda_0 \in (0, \lambda_c)$ with $x_1 = \ln\left( \frac{\beta^2 - 1}{\beta - \gamma} \right)$, there exists $k > 0$ and $\delta > 0$ such that for all $\lambda \in \gU([0, \lambda_0], \delta)$ we have
    \begin{align*}
        g_{\lambda}(\tilde{U}(k)) \subseteq U(x_1, k).
    \end{align*}
\end{lemma}
\begin{proof}
    We divide the proof into three parts to prove this conclusion. In the first part, we deal with sufficiently large $|\re(z)|$ for $z \in \tilde{U}$. In the second part, we provide the proof for real $\lambda$ and $z \in \tilde{U}(k)$ with bounded $|\re(z)|$ based on Lemma \ref{lem:boundary} and invariance of domain for injective continuous map. In the last part, we recall the technique employed in the proof of Lemma \ref{lem:hard-core:complex}, and extend the results for real $\lambda$ to complex $\lambda$ with $z \in \tilde{U}(k)$ and bounded $|\re(z)|$. 
    
    \textbf{(1) Sufficiently large $\re(z)$}
    
    Consider $w = -x + \i y \in \tilde{U}$ with $x \ge \frac{\pi}{4 k}$. 
    Suppose that $\lambda = |\lambda| e^{i \theta}$, $|\lambda| < \lambda_c$ and $k < \frac{\pi}{4 \ln(\lambda_c \beta)}$. Then there holds that $x > \ln(\lambda_c \beta)$, $|\lambda| e^{-x} < \frac{1}{\beta}$ and
    \begin{align*}
        \re(1 + \gamma \lambda e^{w}) &= 1 + \gamma |\lambda| e^{-x} \cos(y + \beta) > 1 - \frac{\gamma}{\beta} > 0, \\
        \re(\beta + \lambda e^{w}) &= \beta + |\lambda| e^{-x} \cos(y + \beta) > \beta - \frac{1}{\beta} > 0.
    \end{align*}
    Therefore we can compute that
    \begin{align*}
        \re \left(g_{\lambda}(w)\right) &= \ln \left\vert \frac{\gamma \lambda e^{w} + 1}{\lambda e^{w} + \beta} \right\vert 
        = \frac{1}{2} \ln \left(\frac{1 + \gamma^2 |\lambda|^2 e^{-2x} + 2 \gamma |\lambda| e^{-x} \cos(y + \theta)}{\beta^2 + |\lambda|^2 e^{-2x} + 2 \beta |\lambda| e^{-x} \cos(y + \theta)}\right), \\
        \im(g_{\lambda}(w)) &= \arg(\gamma |\lambda| e^{-x + i(y + \theta)} + 1) - \arg(|\lambda| e^{-x + i(y + \theta)} + \beta) \\
        &= \arctan\left( \frac{\gamma |\lambda| e^{-x} \sin(y + \theta)}{1 + \gamma |\lambda| e^{-x} \cos(y + \theta)} \right)
        - \arctan\left( \frac{|\lambda| e^{-x} \sin(y + \theta)}{\beta + |\lambda| e^{-x} \cos(y + \theta)} \right) \\
        &= \arctan\left( \frac{(\beta \gamma - 1) |\lambda| e^{-x} \sin(y + \theta)}{\beta + \gamma |\lambda|^2 e^{-2x} + (\beta \gamma + 1)|\lambda| e^{-x} \cos(y + \theta)} \right),
    \end{align*}
    where we have applied $\tan(x - y) = \frac{\tan(x) - \tan(y)}{1 + \tan(x) \tan(y)}$.
    
    Next, note that
    \begin{align*}
        &\quad \frac{\beta^2 + |\lambda|^2 e^{-2x} + 2 \beta |\lambda| e^{-x} \cos(y + \theta)}{1 + \gamma^2 |\lambda|^2 e^{-2x} + 2 \gamma |\lambda| e^{-x} \cos(y + \theta)} \\
        &= \frac{\beta}{\gamma} + \frac{(\beta/\gamma - |\lambda|^2 e^{-2x})(\beta \gamma - 1)}{1 + \gamma^2 |\lambda|^2 e^{-2x} + 2 \gamma |\lambda| e^{-x} \cos(y + \theta)} \\
        &\le \frac{\beta}{\gamma} + \frac{(\beta/\gamma - |\lambda|^2 e^{-2x})(\beta \gamma - 1)}{1 + \gamma^2 |\lambda|^2 e^{-2x} - 2 \gamma |\lambda| e^{-x}} \\
        &= \left( \frac{\beta - |\lambda| e^{-x}}{1 - \gamma |\lambda| e^{-x}} \right)^2 
        < \left( \frac{\beta - 1/\beta}{1 - \gamma /\beta} \right)^2
        = \left( \frac{\beta^2 - 1}{\beta - \gamma} \right)^2,
    \end{align*}
    and
    \begin{align}\label{eq:large-x-r-bound}
    \begin{split}
        &\quad \frac{\beta^2 + |\lambda|^2 e^{-2x} + 2 \beta |\lambda| e^{-x} \cos(y + \theta)}{1 + \gamma^2 |\lambda|^2 e^{-2x} + 2 \gamma |\lambda| e^{-x} \cos(y + \theta)} \\
        &\ge \frac{\beta}{\gamma} + \frac{(\beta/\gamma - |\lambda|^2 e^{-2x})(\beta \gamma - 1)}{1 + \gamma^2 |\lambda|^2 e^{-2x} + 2 \gamma |\lambda| e^{-x}} \\
        &= \left( \frac{\beta + |\lambda| e^{-x}}{1 + \gamma |\lambda| e^{-x}} \right)^2 
        > \left( \frac{\beta + 1/\beta}{1 + \gamma /\beta} \right)^2 > 1,
    \end{split}
    \end{align}
    which means $\re(g_{\lambda}(w)) \in \left(-x_1, -\ln\left(\frac{\beta^2 + 1}{\beta + \gamma}\right)\right)$. 
    
    Furthermore, we have 
    \begin{align*}
        \vert \im(g_{\lambda}(w)) \vert &\le \left\vert\frac{(\beta \gamma - 1) |\lambda| e^{-x} \sin(y + \theta)}{\beta + \gamma |\lambda|^2 e^{-2x} + (\beta \gamma + 1)|\lambda| e^{-x} \cos(y + \theta)}\right\vert \\
        &\le \frac{(\beta \gamma - 1) |\lambda| e^{-x}}{\beta + \gamma |\lambda|^2 e^{-2x} - (\beta \gamma + 1)|\lambda| e^{-x}} \\
        &= \frac{(\beta \gamma - 1) |\lambda| e^{-x}}{(\beta - |\lambda| e^{-x})(1 - \gamma |\lambda| e^{-x})} 
        < \frac{(\beta \gamma - 1) \lambda_c e^{-\frac{\pi}{4 k}}}{(\beta - 1/\beta)(1 - \gamma/\beta)},
    \end{align*}
    where we have used that $\arctan(s) \le s$ for $s \ge 0$. 
    
    Hence, it holds that
    \begin{align*}
        \left\vert \frac{\im(g_{\lambda}(w))}{\re(g_{\lambda}(w))} \right\vert 
        < \frac{(\beta \gamma - 1) \lambda_c e^{-\frac{\pi}{4 k}}}{(\beta - 1/\beta)(1 - \gamma/\beta)\ln\left(\frac{\beta^2 + 1}{\beta + \gamma}\right)}.
    \end{align*}
    Together with $\psi(k) \triangleq k e^{\frac{\pi}{4k}}$ is a decreasing function for $k \in(0, \pi/4)$ and $\lim_{k \to 0^{+}} \psi(k) = + \infty$, we know that
    \begin{align*}
        \left\vert \frac{\im(g_{\lambda}(w))}{\re(g_{\lambda}(w))} \right\vert < k, ~~~ \forall w \in \tilde{U}, |\re(w)| > \frac{\pi}{4 k}. 
    \end{align*}
    holds for any $k < k_1$ for a constant $k_1 > 0$. 
    
    
    \textbf{(2) Real $\lambda$ and Bounded $\re(z)$}
    
    In this part, we will show that there exists $k > 0$ such that
    \begin{align*}
        g_{\lambda} \left(U\left(\frac{\pi}{4k}, k\right)\right) \subseteq \open{U(x_1, k)}. 
    \end{align*}
    
    Consider $w = -x + \i y \in U(\frac{\pi}{4k}, k)$ and $\lambda \in [0, \lambda_0]$. Note that $x \in [0, \frac{\pi}{4 k}]$ and $|y| \le k x < \frac{\pi}{4}$ and 
    \begin{align*}
        \re(1 + \gamma \lambda e^{w}) = 1 + \gamma \lambda e^{-x}\cos(y) > 0, \\
        \re(\beta + \lambda e^{w}) = \beta + \lambda e^{-x} \cos(y) > 0.
    \end{align*}
    Hence, we can define
    \begin{align*}
        r(x, y, k) &\triangleq \re(g_{\lambda}(z)) = \frac{1}{2} \ln \left(\frac{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(y)}{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)}\right), \\
        h(x, y, k) &\triangleq \im(g_{\lambda}(z)) = \arctan\left( \frac{(\beta \gamma - 1) \lambda e^{-x} \sin(y)}{\beta + \gamma \lambda^2 e^{-2x} + (\beta \gamma + 1)\lambda e^{-x} \cos(y)} \right).
    \end{align*}
    Without loss of generality, we assume that $y \ge 0$. 
    
    Note that $r(x, y, k) < 0$ is equivalent to 
    \begin{align*}
        (1 - \gamma^2) \lambda^2 e^{-2x} + (\beta^2 - 1) + 2 (\beta - \gamma) \lambda e^{-x} \cos(y) > 0,
    \end{align*}
    which follows from $\beta > 1 \ge \gamma$ and $\cos(y) > 0$.
    On the other hand, 
    \begin{align*}
        &\quad \frac{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)}{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(y)} - \beta^2 \\
        &= -\frac{(\beta^2\gamma^2 - 1)\lambda^2 e^{-2x} + 2\beta(\beta\gamma - 1)\lambda e^{-x} \cos(y)}{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(y)} < 0,
    \end{align*}
    where we have recalled that $\cos(y) > 0$.
    Therefore $r(x, y, k) > -\ln(\beta) > -\ln\left( \frac{\beta^2 - 1}{\beta - \gamma} \right) = -x_1$.
    
    Therefore, we just need to choose $k \in (0, k_1)$ such that 
    \[h(x, y, k) < - k r(x, y, k), ~~~\text{ for } x \in [0, \frac{\pi}{4k}], ~y \in [0, k x], \] 
    where $k_1$ is defined in previous part. 
    Choose $x_0 \ge \max\{1, \ln(\lambda \gamma)\}$ such that
    \begin{align*}
        x_0 e^{-x_0} \le \frac{\beta \ln(\beta/2) }{(\beta\gamma - 1)\lambda}. 
    \end{align*}
    Then for $x \in [x_0, \frac{\pi}{4 k}]$ and $y \in [0, k x]$, we have 
    \begin{align*}
        -r(x, y, k) &= \frac{1}{2} \ln \left(\frac{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)}{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(y)}\right) \\
        &> \frac{1}{2} \ln \left(\frac{\beta^2}{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x}}\right) \\
        &\ge \ln \left(\frac{\beta}{1 + \gamma \lambda e^{-x_0}}\right)
        \ge \ln(\beta/2),
    \end{align*}
    where the last inequality is according to $e^{-x_0} \le \frac{1}{\lambda\gamma}$. 
    Therefore, we can conclude that
    \begin{align*}
        h(x, y, k) &\le \frac{(\beta \gamma - 1) \lambda e^{-x} \sin(y)}{\beta + \gamma \lambda^2 e^{-2x} + (\beta \gamma + 1)\lambda e^{-x} \cos(y)} \\
        &\le \frac{(\beta\gamma - 1) \lambda e^{-x} k x}{\beta} \\
        &\le \frac{(\beta\gamma - 1) \lambda e^{-x_0} k x_0}{\beta} \\
        &\le k \ln(\beta / 2) < -k r(x, y, k),
    \end{align*}
    where we have used that $\arctan(s) \le s, \sin(s) \le s$ for $s \ge 0$ and the function $\psi(s) = x e^{-x}$ is decreasing when $x \ge 1$. 
    
    Now we only need to prove that $g_{\lambda}(U(x_0, k)) \subseteq \open{U(x_1, k)}$. 
    By Lemma \ref{lem:boundary} and $g_{\lambda}$ is injective and holomorphic on $\{z \in \sC: |\im(z)| \le \pi/4\}$, we know that
    \begin{align*}
        \partial g_{\lambda}(U(x_0, k)) = g_{\lambda}(\partial U(x_0, k)).
    \end{align*}
    Moreover, note that
    \begin{align*}
        h(x, y, k) \le \frac{(\beta \gamma - 1) \lambda e^{-x} \sin(y)}{\beta + \gamma \lambda^2 e^{-2x} + (\beta \gamma + 1)\lambda e^{-x} \cos(y)} 
        &\le \frac{(\beta \gamma - 1) \lambda_0}{\beta},
    \end{align*}
    which implies that $g_{\lambda}(\hat{U}(k))$ is bounded. Consequently, it is enough to check that for $x \in [0, x_0]$ 
    \begin{align*}
        H(x, k) &\triangleq -k r(x, k x, k) - h(x, k x, k) \\
        &= \frac{k}{2} \ln \left(\frac{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(k x)}{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(k x)}\right) - \arctan\left( \frac{(\beta \gamma - 1) \lambda e^{-x} \sin(k x)}{\beta + \gamma \lambda^2 e^{-2x} + (\beta \gamma + 1)\lambda e^{-x} \cos(k x)} \right) > 0.
    \end{align*}
    
    Note that
    \begin{align*}
        \frac{\partial H(x, k)}{\partial k} \Bigg\vert_{k = 0} = \ln \left(\frac{\beta + \lambda  e^{-x}}{\gamma \lambda e^{- x}+ 1}\right)-\frac{\lambda  e^x x (\beta  \gamma -1)}{\left(\lambda +\beta  e^x\right) \left(\gamma  \lambda +e^x\right)} \triangleq G(x),
    \end{align*}
    and 
    \begin{align*}
        G'(x) = \frac{\lambda  e^x x (\beta  \gamma -1) \left(\beta  e^{2 x}-\gamma  \lambda ^2\right)}{\left(\lambda +\beta  e^x\right)^2 \left(\gamma  \lambda +e^x\right)^2}.
    \end{align*}
    If $\lambda \le \sqrt{\frac{\beta}{\gamma}}$, then $G'(x) \ge 0$ for all $x \ge 0$. Hence 
    \[G(x) \ge G(0) = \ln\left(\frac{\beta + \lambda}{\gamma \lambda + 1}\right) \ge \ln\left(\frac{\beta + \sqrt{\beta/\gamma}}{\gamma \sqrt{\beta/\gamma} + 1} \right) = \frac{1}{2} \ln(\beta/\gamma). \]
    If $\lambda \ge \sqrt{\frac{\beta}{\gamma}}$, then $G'(x) < 0$ for $x \in [0, \ln(\lambda \sqrt{\gamma/\beta}))$ and $G'(x) > 0$ for $x > \ln(\lambda \sqrt{\gamma/\beta})$. Therefore, we have
    \begin{align*}
        G(x) &\ge G(\ln(\lambda \sqrt{\gamma/\beta})) \\
        &= \ln\left( \frac{\beta + \sqrt{\beta/\gamma}}{\gamma \sqrt{\beta/\gamma} + 1} \right) - \frac{(\beta\gamma - 1)\lambda^2 \sqrt{\gamma/\beta} \ln(\lambda\sqrt{\gamma/\beta})}{(\lambda + \beta \lambda\sqrt{\gamma/\beta})(\gamma \lambda + \lambda \sqrt{\gamma/\beta})} \\
        &= \frac{1}{2} \ln(\beta/\gamma) - \frac{(\beta\gamma - 1) \ln(\lambda \sqrt{\gamma/\beta})}{(1 + \sqrt{\beta\gamma})^2} \\
        &= \frac{\sqrt{\beta\gamma}}{\sqrt{\beta\gamma} + 1} \ln(\beta/\gamma) - \frac{\sqrt{\beta\gamma} - 1}{\sqrt{\beta\gamma} + 1} \ln(\lambda).
    \end{align*}
    Together with $\lambda \le \lambda_0 < \lambda_c = \left( \frac{\beta}{\gamma} \right)^{\frac{\sqrt{\beta\gamma}}{\sqrt{\beta\gamma} - 1}}$, we have $G(x) > \eps$ for any $x \ge 0$ and $\lambda \in [0, \lambda_0]$. Then there exist $k_2 > 0$ such that for all $k \le k_1$ and $x \in [0, x_0]$, we have
    \begin{align*}
        \frac{\partial H(x, k)}{\partial k} > \frac{\eps}{2}.
    \end{align*}
    Then recalling that $H(x, 0) = 0$, it holds that
    \begin{align*}
        H(x, k_2) = \int_{0}^{k_2} \frac{\partial H(x, k)}{\partial k} d k \ge \frac{\delta k_2}{2} > 0.
    \end{align*}

    \textbf{Complex $\lambda$ and Bounded $\re(z)$}
    
    In previous part, we prove that there exists $k > 0$ such that for all $\lambda \in [0, \lambda_0]$
    \begin{align}\label{eq:ferro:complex}
            g_{\lambda} \left(U\left(\frac{\pi}{4k}, k\right)\right) \subseteq \open{U(x_1, k)}. 
    \end{align}
    Now fix $k$, then $U\left(\frac{\pi}{4k}, k\right)$ is a compact set. 
    Then following from the proof of Lemma \ref{lem:hard-core:complex}, there exists $\delta > 0$ such that Equation (\ref{eq:ferro:complex}) also holds for all $\lambda \in \gU([0, \lambda_0], \delta)$.
    
\end{proof}

\subsection{Negative Weight $\lambda$}
In this section, we prove that following result.
\begin{lemma}\label{lem:ferro:real:negative}
    For $\beta > 1 \ge \gamma$ and $\lambda_0 \in (-1/\gamma, 0)$ with $x_1 = \ln\left( \frac{\beta^2 - 1}{\beta - \gamma} \right)$, there exists $k > 0$ and $\delta > 0$ such that for all $\lambda \in \gU([\lambda_0, 0], \delta)$ we have
    \begin{align*}
        g_{\lambda}(\tilde{U}(k)) \subseteq U(x_1, k).
    \end{align*}
\end{lemma}
\begin{proof}
    We also divide the proof into three parts to prove this conclusion. 
    
    \textbf{(1) Sufficiently large $\re(z)$}
    
    Consider $w = -x + \i y \in \tilde{U}$ with $x \ge \frac{\pi}{4 k}$. 
    Suppose that $\lambda = |\lambda| e^{i \theta}$, $|\lambda| < 1/\gamma$ and $k < \frac{\pi}{4 \ln(\beta/\gamma)}$. Following from part (1) of the proof of Lemma \ref{lem:ferro:real}, we know that 
    \begin{align*}
        \re(g_{\lambda}(w)) &\in \left(-x_1, -\ln\left(\frac{\beta^2 + 1}{\beta + \gamma}\right)\right), \\
        \left\vert \frac{\im(g_{\lambda}(w))}{\re(g_{\lambda}(w))} \right\vert 
        &< \frac{(\beta - 1/\gamma) e^{-\frac{\pi}{4 k}}}{(\beta - 1/\beta)(1 - \gamma/\beta)\ln\left(\frac{\beta^2 + 1}{\beta + \gamma}\right)} < k, ~~~\text{ for } k < k_1. 
    \end{align*}
    
    \textbf{(2) Real $\lambda$ and Bounded $\re(z)$}
    
    In this part, we will show that there exists $k > 0$ such that
    \begin{align*}
        g_{\lambda} \left(U\left(\frac{\pi}{4k}, k\right)\right) \subseteq \open{U(x_1, k)}. 
    \end{align*}
    Consider $w = -x + \i y \in U(\frac{\pi}{4k}, k)$ and $\lambda \in [\lambda_0, 0]$. Note that $x \in [0, \frac{\pi}{4 k}]$ and $|y| \le k x < \frac{\pi}{4}$ and 
    \begin{align*}
        \re(1 + \gamma \lambda e^{w}) = 1 + \gamma \lambda e^{-x}\cos(y) \ge 1 - \gamma |\lambda| > 0, \\
        \re(\beta + \lambda e^{w}) = \beta + \lambda e^{-x} \cos(y) \ge \beta - |\gamma| > 0.
    \end{align*}
    Hence, we can define
    \begin{align*}
        r(x, y, k) &\triangleq \re(g_{\lambda}(z)) = \frac{1}{2} \ln \left(\frac{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(y)}{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)}\right), \\
        h(x, y, k) &\triangleq |\im(g_{\lambda}(z))| = \arctan\left( \frac{(\beta \gamma - 1) |\lambda| e^{-x} \sin(y)}{\beta + \gamma \lambda^2 e^{-2x} + (\beta \gamma + 1)\lambda e^{-x} \cos(y)} \right).
    \end{align*}
    Without loss of generality, we assume that $y \ge 0$. 
    Note that
    \begin{align*}
        &\quad \frac{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(y)}{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)} \\
        &= \frac{\gamma}{\beta} - \frac{(1 - \gamma/\beta \lambda^2 e^{-2x})(\beta \gamma - 1)}{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)} \\
        &\le \frac{\gamma}{\beta} - \frac{(1 - \gamma/\beta \lambda^2 e^{-2x})(\beta \gamma - 1)}{\beta^2 + \lambda^2 e^{-2x}} \\
        &= \frac{1 + \gamma^2 \lambda^2 e^{-2 x}}{\beta^2 + \lambda^2 e^{-2 x}} \le \frac{2}{\beta^2 + 1/\gamma^2} < 1,
    \end{align*}
    where we have noticed that $\lambda e^{-x} \in (-1/\gamma, 0]$.
    
    On the other hand, 
    \begin{align*}
        &\quad \frac{1 + \gamma^2 \lambda^2 e^{-2x} + 2 \gamma \lambda e^{-x} \cos(y)}{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)} \\
        &= \frac{\gamma}{\beta} - \frac{(1 - \gamma/\beta \lambda^2 e^{-2x})(\beta \gamma - 1)}{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x} \cos(y)} \\
        &\ge \frac{\gamma}{\beta} - \frac{(1 - \gamma/\beta \lambda^2 e^{-2x})(\beta \gamma - 1)}{\beta^2 + \lambda^2 e^{-2x} + 2 \beta \lambda e^{-x}} \\
        &= \left(\frac{1 + \gamma \lambda e^{-x}}{\beta + \lambda e^{-x}}\right)^2 \le \frac{1}{\beta^2} < 1,
    \end{align*}
    where we have recalled that $\cos(y) > 0$.
    Therefore $r(x, y, k) > -\ln(\beta) > -\ln\left( \frac{\beta^2 - 1}{\beta - \gamma} \right) = -x_1$.
\end{proof}



We here choose $U(x_1, x_0, k)$ where $x_0 \le 0$ for finding $U_{\lambda}$. The key step for finding $x_0, k$ is to verify that for $z = -x + \i k (x_0 + x) \in \partial U(x_1, x_0, k)$ there holds
\begin{align*}
    &k(x_0 - \re(g_{\lambda}(d z))) - |\im(g_{\lambda}(d z))| > 0, ~~~~~~\text{i.e.,} \\
    &H(x, k) \triangleq k\left(x_0 + \frac{1}{2}\ln\left( \frac{\beta^2 + \lambda^2 e^{-2 d x} + 2\beta \lambda e^{-d x} \cos(k d (x_0 + x))}{1 + \gamma^2 \lambda^2 e^{-2 d x} + 2 \gamma \lambda e^{-d x} \cos(k d (x_0 + x))} \right)\right) \\
    &- \arctan\left( \frac{(\beta\gamma - 1)|\lambda| e^{- d x} \sin(k d (x_0 + x))}{\beta + \gamma \lambda^2 e^{-2 d x} + (\beta\gamma + 1)\lambda e^{-d x} \cos(k d (x_0 + x))} \right) > 0,
\end{align*}
and
\begin{align*}
    G(x) \triangleq \frac{\partial H(x, k)}{\partial k} \Bigg\vert_{k = 0} = x_0 + \ln \left(\frac{\beta + \lambda  e^{-d x}}{1 + \gamma \lambda e^{-d x}}\right) + \frac{(\beta \gamma -1) \lambda  e^{-d x} d\left(x_0+x\right)}{(\beta + \lambda  e^{-d x})(1 + \gamma \lambda e^{- d x})} > 0.
\end{align*}

Note that 
\begin{align*}
    G'(x) = -\frac{d   (\beta  \gamma -1) \lambda e^{-d x} \left(-2 (\beta  \gamma +1) \lambda e^{-d x}+\beta (d (x+x_0)-2)-\gamma (d (x+x_0)+2) \lambda ^2 e^{-2 d x}\right)}{\left(\beta +\lambda e^{-d x} \right)^2 \left(\gamma  \lambda e^{-d x} +1\right)^2}.
\end{align*}

Consider following function
\begin{align*}
    \Psi(x) &\triangleq -2 (\beta  \gamma +1) \lambda e^{-d x}+\beta (d (x+x_0)-2)-\gamma (d (x+x_0)+2) \lambda ^2 e^{-2 d x} \\
    &= d(x + x_0) (\beta - \gamma \lambda^2 e^{-2 d x}) - 2 (\beta + \lambda e^{-d x})(1 + \gamma \lambda e^{-d x}).
\end{align*}
Assume that
\begin{align*}
    |\lambda| e^{(\Delta - 1) x_0} < \frac{1}{\gamma}.
\end{align*}
Then we have
\begin{align*}
    \Psi'(x) &= d \left(\beta +2 \lambda  (\beta  \gamma +1) e^{-d x}+\gamma  \lambda ^2 e^{-2 d x} (2 d (x+x_0)+3)\right), \\
    \Psi''(x) &= -2 d^2 \lambda  e^{-d x} \left((\beta  \gamma +1) +2 \gamma  (d (x+x_0)+1) \lambda e^{- d x} \right), \\
    \psi(x) &\triangleq (\beta  \gamma +1) +2 \gamma  (d (x+x_0)+1) \lambda e^{- d x}, \\
    \psi'(x) &= -2 \gamma  d^2 \lambda  e^{-d x} (x+x_0) \ge 0.
\end{align*}

Consequently, there holds
\[\Psi''(x) \ge 2 d^2 |\lambda|  e^{-d x} \left((\beta  \gamma +1) +2 \gamma \lambda e^{- d x_0} \right) > 0, \]
which means $\Psi(x)$ is strictly convex on $[-x_0, +\infty)$. Together with 
\begin{align*}
    \Psi(-x_0) &= -2 (\beta + \lambda e^{d x_0})(1 + \gamma \lambda e^{d x_0}) < 0, \\
    \Psi(x) &\to + \infty, \text{  for  } x \to +\infty,
\end{align*}
therefore, we can conclude that $\psi(x) = 0$ has unique solution on $[-x_0, +\infty)$, and denote this solution to be $s(x_0, \lambda)$. Moreover, $\psi(x) < 0$ and $G'(x) < 0$ when $x < s(x_0, \lambda)$, and $\psi(x) > 0$ and $G'(x) > 0$ when $x > s(x_0, \lambda)$. Hence we just need to verify that
\begin{align*}
    G(x) \ge G(s(x_0, \lambda)) &= x_0 + \ln \left(\frac{\beta + \lambda  e^{-d s}}{1 + \gamma \lambda e^{-d s}}\right) + \frac{(\beta \gamma -1) \lambda  e^{-d s} d\left(x_0+s\right)}{(\beta + \lambda  e^{-d s})(1 + \gamma \lambda e^{- d s})} \\
    &= x_0 + \ln \left(\frac{\beta + \lambda  e^{-d s}}{1 + \gamma \lambda e^{-d s}}\right) + \frac{2(\beta \gamma -1) \lambda e^{-d s}}{\beta - \gamma \lambda^2 e^{-2 d s}} > 0,
\end{align*} 
for all $d \le \Delta - 1$.

Letting $\hat{s} = \lambda e^{- d s}$, then we have $\hat{s} > \lambda e^{d x_0} > -\frac{1}{\gamma} $ and
\begin{align*}
    \frac{2(\beta + \hat{s})(1 + \gamma \hat{s})}{\beta - \gamma \hat{s}^2} = d(s + x_0), \\
    \hat{s} \exp\left( \frac{2(\beta + \hat{s})(1 + \gamma \hat{s})}{\beta - \gamma \hat{s}^2} \right)  = \lambda e^{d x_0}.
\end{align*}

Define
\begin{align*}
    F(s) =  s \exp\left( \frac{2(\beta + s)(1 + \gamma s)}{\beta - \gamma s^2} \right).
\end{align*}
And note that
\begin{align*}
    F'(s) = \exp\left(\frac{2 (\beta +s) (\gamma  s+1)}{\beta -\gamma  s^2}\right) \frac{ (\beta +2 \beta\gamma s + \gamma s^2) (\beta + 2 s + \gamma s^2)}{\left(\beta -\gamma  s^2\right)^2}.
\end{align*}
Observe that $F'(s) < 0$ for $s \in \left(-\frac{1}{\gamma}, s_0\right)$ and $F'(s) > 0$ for $s \in (s_0, 0]$ where $s_0 = -\beta + \sqrt{\frac{\beta(\beta\gamma - 1)}{\gamma}}$. Together with $F(-1/\gamma) = -1/\gamma < \lambda e^{d x_0}$, we know that $\hat{s} > s_0$. 


==> hard-core.tex <==
\section{Hard-Core Models}
The independence polynomial of a graph $G$ is defined as 
\begin{align*}
    Z_{G} (\lambda) = \sum_{I \in \gI(G)} \lambda^{|I|}. 
\end{align*}

For a graph $G$, define
\begin{align}
    R^{\lambda}(G, v) = \frac{\lambda Z_{G - \gN(v)}(\lambda)}{Z_{G - v}(\lambda)},
\end{align}
where $\gN(v) = \{v\} \cup \{u: u \sim v\}$.
Note that 
\begin{align*}
    Z_{G}(\lambda) = Z_{G - v}(\lambda) + \lambda Z_{G - \gN(v)}(\lambda),
\end{align*}
which implies that 
\[Z_{G}(\lambda) = 0 \iff R^{\lambda}(G, v) = -1.\]

Following lemma implies that it is enough to consider the zero-freeness of $Z_{G}$ for trees.   
\begin{lemma}[{\cite{bencs2018trees}}]
    For every graph $G$ with maximum degree at most $\Delta$ there exists a tree $T_G$ with maximum degree at most $\Delta$ such that $Z_{G}(\lambda)$ divides $Z_{T_G}(\lambda)$ as a polynomial.
\end{lemma}

Given a tree $T$ rooted at $v$, and assume that $u_1, \dots, u_d$ are the neighbours of $v$ and $T_i$ are subtrees rooted at $u_i$ for $i \in [d]$. It can be shown that
\begin{align*}
    R^{\lambda}(T, v) = \frac{\lambda}{\prod_{i=1}^d \left(1 + R^{\lambda}(T_i, u_i)\right)}.
\end{align*}

\begin{definition}
    We say $\lambda \in \sC$ satisfies $d$-complex-contraction property for hard-core models if there is an open domain $F_{\lambda} \subseteq \sC$ such that 
    \begin{enumerate}
        \item $0 \in F_{\lambda}, -1 \notin \overline{F_{\lambda}}$,
        \item $f_{\lambda, d}(z_1, \dots, z_{d}) \in F_{\lambda}$ for any $z_i \in F_{\lambda}, i = 1, \dots, d$, where the map $f_{\lambda, d}$ is defined as
        \begin{align*}
        f_{\lambda, d}(z_1, \dots, z_d) = \frac{\lambda}{\prod_{i=1}^d (1 + z_i)}.
    \end{align*}
    \end{enumerate}
\end{definition}

We remark here that $f_{\lambda, \hat{d}}(z_1, \dots, z_{\hat{d}}) = f_{\lambda, d}(z_1, \dots, z_{\hat{d}}, 0, \dots, 0)$ for any $\hat{d} < d$. Based on $0 \in F_{\lambda}$, if $\lambda$ satisfies $d$-complex-contraction property, then $\lambda$ also satisfies $\hat{d}$-complex-contraction property for any $\hat{d} < d$.

Following lemma shows the equivalence between $(\Delta -1)$-complex-contraction and absence of zeros for hard-core models. 
\begin{lemma}[{\cite{bencs2018note}}]
    If $\lambda$ satisfies $(\Delta-1)$-complex-contraction, then $Z_{G}(\lambda) \neq 0$ for any graph $G$ with maximum degree $\Delta$.
\end{lemma}

\subsection{Complex Contraction}
In this section, we present a direct proof of complex contraction for Hard-Core Model and prove following statement. 
\begin{thm}
    Suppose that $\lambda_0 \in \left( -\frac{(\Delta - 1)^{\Delta - 1}}{\Delta^{\Delta}}, \frac{(\Delta - 1)^{\Delta - 1}}{(\Delta - 2)^{\Delta}} \right)$, there exists $\delta > 0$ such that for any $\lambda \in \gU([0, \lambda_0], \delta)$ we have $(\Delta - 1)$-complex-contraction property holds for $\lambda$. 
\end{thm}

In \cite{peters2019conjecture, shao2019contraction}, the authors showed the complex contraction property by proving correlation decay for real $\lambda$ and (uniformly) continuity of the map $f_{\lambda, d}$ with respect to $\lambda$. We point out that finding a ``good'' potential function $\phi$ plays an important role in their proof. 
With a potential function $\phi$, we define
\begin{align*}
    f^{\phi}_{\lambda, d}(w_1, \dots, w_d) \triangleq \phi \left( f_{\lambda, d}(\phi^{-1}(w_1), \dots, \phi^{-1}(w_d)) \right).
\end{align*}
In \cite{peters2019conjecture}, the authors employed a potential function 
\[\phi(x) = \log(1 + c \log(1 + x)),\] 
where $c$ is depend on $\Delta$, and in \cite{shao2019contraction}, the authors applied a potential function \[\phi(x) = \int_{1}^x \frac{1}{\sqrt{t(t+1)}} d t\]
to show that for all real $\lambda \in [0, \lambda_0]$, $d \le \Delta - 1$, 
\[\Norm{\nabla f^{\phi}_{\lambda, d}(\vw)}_1 < 1 - \eta, ~~~ \vw \in J^d,\] 
where $\eta > 0$ is a constant and $J$ is an real interval.

Following we will introduce our method without depending on well-designed potential functions. At first, we note that the product of same regions is often not easy to find. 
Hence we consider a potential function $\phi(z) = - \ln(1 + z)$, which allows us to deal with the sum of same regions. 
Actually we have
\begin{align}
    f^{\phi}_{\lambda, d}(w_1, \dots, w_d) = \phi \left( f_{\lambda, d}(\phi^{-1}(w_1), \dots, \phi^{-1}(w_d)) \right) = - \ln\left(1 + \lambda e^{\sum_{i=1}^d w_i}\right). 
\end{align}
Observe that for convex region $U$ it holds that
\begin{align*}
    \left\{\sum_{i=1}^d w_i: \vw \in U^d\right\} = d U \triangleq \{d w: w \in U\}.
\end{align*}

Now our goal is to find a convex and open region $U_{\lambda}$ as follows.
\begin{lemma}
    For $\lambda \in \sC$, if there exists convex and open region $U_{\lambda} \subseteq \{z: |\im{z}| < \pi \}$ such that 
    \begin{enumerate}
        \item $0 \in U_{\lambda}$, $-1 \notin \overline{\phi^{-1}(U_{\lambda})}$,
        \item $g_{\lambda, \Delta - 1}(U_{\lambda}) \subseteq U_{\lambda}$ where
        $
            g_{\lambda, d}(z) = - \ln(1 + \lambda e^{d z}),
        $
    \end{enumerate}
    then $\lambda$ satisfies $(\Delta-1)$-complex-contraction property.
\end{lemma}
\begin{proof}
    Note that $\phi$ is a bijection between $\sC \backslash (-\infty, -1]$ and $\{z: |\im{z}| < \pi \}$. Thus we can set $F_{\lambda} = \phi^{-1}(U_{\lambda})$ which is a open region based on open mapping theorem.
\end{proof}

We choose following class of isosceles triangles for finding $U_{\lambda}$. 
\begin{align}
    U(x_0, x_1, k) = \{z: \re(z) \in (x_1, x_0), |\im(z)| < k (x_0 - \re(z)) \}, 
\end{align}
where $x_1 < 0, x_0 > 0, k > 0$.
It is clear that $0 \in U(x_0, x_1, k)$. Further, recall that $\phi$ is a bijection between $\sC \backslash (-\infty, -1]$ and $\{z: |\im{z}| < \pi \}$. Hence $-1 \notin \phi^{-1}(U(x_0, x_1, k))$ for $k < \frac{\pi}{x_0 - x_1}$. 

% Now, we picture the region $g_{\lambda, \Delta-1}(U(x_0, x_1, k))$ as follows. 
\begin{lemma}\label{lem:hard-core:real}
    There exists $x_0, x_1, k$ such that for all $\lambda \in [0, \lambda_0]$ we have
    \begin{align*}
        \overline{g_{\lambda, \Delta-1}(U(x_0, x_1, k))} \subseteq U(x_0, x_1, k).
    \end{align*}
\end{lemma}
\begin{proof}
    Let $d = \Delta-1$. 
    We prove the result in two cases $\lambda_0 > 0$ and $\lambda_0 < 0$ respectively. 
    
    \textbf{(1) The case $\lambda_0 > 0$. }
    
    Suppose that $k < k_0 \triangleq \frac{\pi}{2 d (x_0 - x_1)}$ and $\lambda \in (0, \lambda_0]$. 
    Then for $z \in U(x_0, x_1, k)$, we have $|\im (d z)| < \frac{\pi}{2}$ which implies that 
    % $h(z) = e^{d z}$ is injective on $\overline{U(x_0, x_1, k)}$ and
    \begin{align*}
        \re (\lambda e^{d z}) = \lambda e^{d \re(z)} \cos(d \im(z)) > 0.
    \end{align*}
    % Consequently, $g_{\lambda, d}$ is injective and holomorphic on $\overline{U(x_0, x_1, k)}$. 
    % Then by Lemma \ref{lem:boundary}, we have 
    % \begin{align*}
    %     \partial g_{\lambda, \Delta-1}(U(x_0, x_1, k)) = g_{\lambda, \Delta-1}(\partial U(x_0, x_1, k)).
    % \end{align*}
    % By invariance of domain, the domain of $g_{\lambda, \Delta-1}(U(x_0, x_1, k))$ is also simply connected. 
    % Together with $g_{\lambda, \Delta-1}(0) = -\ln(1 + \lambda) \in U(x_0, x_1, k)$ when $x_1 \le -\ln(1 + \lambda)$, we only need to ensure that
    % \begin{align*}
    %     g_{\lambda, \Delta-1}(\partial U(x_0, x_1, k)) \subseteq U(x_0, x_1, k).
    % \end{align*}
    
    By symmetry of $U(x_0, x_1, k)$, we just need to consider $z \in \partial U(x_0, x_1, k)$ with $\im(z) \ge 0$. 
    For $z = -x + \i y \in \partial U(x_0, x_1, k)$ with $x \in [-x_0, -x_1]$ and $y \in [0, k(x_0 + x)]$, define
    \begin{align*}
        r(x, y) &\triangleq \re(g_{\lambda, d}(z)) = -\frac{1}{2} \ln\left( 1 + \lambda^2 e^{-2 d x} + 2 \lambda e^{-d x} \cos(d y) \right), \\
        h(x, y) &\triangleq |\im(g_{\lambda, d}(z))| = \arctan\left( \frac{\lambda e^{-d x} \sin(d y)}{1 + \lambda e^{-d x} \cos(d y)} \right).
    \end{align*}
    
    Note that $d k y < \frac{\pi}{2}$, we have
    \begin{align*}
        r(x, y) \le - \frac{1}{2} \ln(1 + \lambda^2 e^{-2 d x}) \le 0,
    \end{align*}
    and
    \begin{align*}
        r(x, y) \ge -\frac{1}{2} \ln\left( 1 + \lambda^2 e^{-2 d x} + 2 \lambda e^{- d x}\right) = -\ln\left(1 + \lambda e^{- d x}\right) \ge - \ln\left( 1 + \lambda_0 e^{d x_0} \right).
    \end{align*}
    Hence, to ensure $r(x, y) \in (x_1, x_0)$, it is enough to set 
    \begin{align}\label{def:hard-core:x1}
        x_1 = - \ln\left( 1 + \lambda_0 e^{d x_0} \right) - 2.
    \end{align} 
    
    Next, we need to determine $x_0, k$ to ensure that
    \begin{align*}
        h(x, y) < k(x - r(x, y)),
    \end{align*}
    which implies that $\overline{g_{\lambda, d}(U(x_0, x_1, k))} = g_{\lambda, d}(\overline{U(x_0, x_1, k)}) \subseteq U(x_0, x_1, k)$. 
    Define
    \begin{align*}
        J(x, y, k) &\triangleq k(x_0 - r(x, y)) - h(x, y) \\
        &= k \left(x_0 + \frac{1}{2} \ln\left( 1 + \lambda^2 e^{-2 d x} + 2 \lambda e^{-d x} \cos(d y) \right)\right) - \arctan\left( \frac{\lambda e^{-d x} \sin(d y)}{1 + \lambda e^{-d x} \cos(d y)} \right).
    \end{align*}
    Note that 
    \begin{align*}
        \frac{\partial J(x, y, k)}{\partial y} = -\frac{ d \lambda e^{-dx} (\lambda e^{-dx} + \cos(d y) + k \sin(d y))}{1 + \lambda^2 e^{-2dx} + 2 \lambda e^{-dx} \cos(d y))} < 0.
    \end{align*}
    Therefore, we just need to ensure that 
    \begin{align}\label{def:hard-core:H}
        H(x, k) \triangleq J(x, k(x_0 + x), k) > 0.
    \end{align}
    
    \begin{claim}\label{claim:hard-core:H}
        If \[\frac{\partial H(x, k)}{\partial k} \Bigg\vert_{k = 0} > 0\] holds for all $x \in [-x_0, -x_1]$, then there exists $k > 0$ such that $H(x, k) > 0$ for all $x \in [-x_0, -x_1]$.
    \end{claim}
    \begin{proof}
        Let 
        \begin{align*}
            \hat{H}(x, \hat{k}) \triangleq \frac{\partial H(x, k)}{\partial k} \Bigg\vert_{k = \hat{k}}.
        \end{align*}
        It is easily to check that $\hat{H}(x, \hat{k})$ is continuous on $[-x_0, -x_1] \times [0, k_0]$. 
        
        If for any $k_n = \frac{1}{n}$, there exists $x_n \in [-x_0, -x_1]$ such that $H(x_n, k_n) \le 0$. 
        Then by $H(x_n, 0) = 0$ and mean value theorem, there exists $\xi_n \in (0, k_n)$ such that $\hat{H}(x, \xi_n) \le 0$. 
        On the other hand, there exists $\{n_m\}_{m \ge 1}$ such that $\lim_{m \to \infty} x_{n_m} = \hat{x} \in [-x_0, -x_1]$. By continuity of $\hat{H}$, we have
        \begin{align*}
            \hat{H}(\hat{x}, 0) = \lim_{m \to \infty} \hat{H}(x_{n_m}, \xi_{n_m}) \le 0,
        \end{align*}
        which leads to a contradiction. 
    \end{proof}
    
    Based on Claim \ref{claim:hard-core:H}, we consider following function
    \begin{align*}
        G(x) \triangleq \frac{\partial H(x, k)}{\partial k} \bigg\vert_{k = 0} = x_0 - \frac{d(x + x_0) \lambda e^{-d x}}{1 + \lambda e^{-d x}} +  \ln\left( 1 + \lambda e^{- d x} \right).
    \end{align*}
    
    % Let 
    % \begin{align}
    %     x_0 = \frac{2}{d-1} - \ln \left(\frac{d}{d-1} \right).
    % \end{align}
    % By $\ln(1 + x) \le x$, we have $\ln(d/(d-1)) \le 1/(d-1)$ and $x_0 \ge \frac{1}{d-1}$.
    
    Now observe that 
    \begin{align*}
        G'(x) = \frac{d \lambda e^{-d x}( d(x + x_0) - 2 (1 + \lambda e^{-d x}))}{(1 + \lambda e^{- d x})^2}.
    \end{align*}
    Denote 
    \begin{align*}
        \hat{G}(x) \triangleq d(x + x_0) - 2(1 + \lambda e^{- d x}).
    \end{align*}
    There holds
    \begin{align*}
        \hat{G}(-x_0) &< 0, \\
        \hat{G}(-x_1) &= d(x_0 - x_1) - 2 (1 + \lambda e^{d x_1}) \\
        &> d x_0 + 2 d - 2 - 2 \lambda e^{-2 d} \\
        &> d x_0 + 2 (d - 1) - \frac{2}{d - 1} \left(\frac{d}{e^2(d-1)} \right) \\
        &\ge d x_0 + 2 (d - 1) - 2 > 0,
    \end{align*}
    where the first inequality is according to $x_1 < -2$ which comes from the definition of $x_1$ in Equation (\ref{def:hard-core:x1}), the second inequality follows from $\lambda \le \lambda_0 < \frac{d^d}{(d-1)^{d+1}}$, and the last inequality is due to $\frac{d}{e^2(d - 1)} < 1$ for $d \ge 2$. 
    
    Then, together with $\hat{G}$ is strictly increasing, we know that there exists $s \in (-x_0, -x_1)$ such that $\hat{G}(s) = 0$, i.e.,
    \begin{align}\label{def:hard-core:s}
        d(s + x_0) = 2(1 + \lambda e^{-d s}).
    \end{align}
    Moreover, we have $G'(x) \le 0$ on $[-x_0, s]$ and $G'(x) \ge 0$ on $[s, -x_1]$ which implies that $G(x) \ge G(s)$.  
    
    Now we set 
    \begin{align}\label{def:hard-core:x0}
        x_0 = \frac{2}{d - 1} - \frac{1}{d} \ln((d-1)\lambda_0).
    \end{align}
    
    \begin{claim}\label{claim:hard-core:s}
        For $x_0$ defined in Equation (\ref{def:hard-core:x0}), we have
        \begin{align*}
            \lambda e^{-d s} \le \frac{1}{d - 1}.
        \end{align*}
    \end{claim}
    \begin{proof}
        Denote $\hat{s} = \lambda e^{-d s}$. Then by Equation (\ref{def:hard-core:s}), we have
        \begin{align*}
            \hat{s} e^{2 \hat{s}} &= \lambda e^{2 \hat{s} - d s} = \lambda e^{d x_0 - 2} \\
            &= \lambda \exp\left( \frac{2 d}{d - 1} - \ln((d-1)\lambda_0) - 2 \right) \\
            &= \frac{\lambda}{(d-1)\lambda_0} e^{\frac{2}{d-1}} \le \frac{1}{d-1} e^{\frac{2}{d-1}}.
        \end{align*}
        Note that the function $\psi(s) = s e^{2s}$ strictly increasing when $s > 0$, hence we have $\hat{s} \le \frac{1}{d-1}$.
    \end{proof}
    
    Based on Claim \ref{claim:hard-core:s}, we have
    \begin{align*}
        G(x) \ge G(s) &= x_0 - \frac{d(s + x_0) \lambda e^{-d s}}{1 + \lambda e^{-d s}} + \ln\left(1 + \lambda e^{-d s}\right) \\
        &= x_0 - 2 \lambda e^{-d s} + \ln\left(1 + \lambda e^{-d s}\right) \\
        &\ge x_0 - \frac{2}{d-1} + \ln\left(1 + \frac{1}{d-1}\right) \\
        &= - \frac{1}{d} \ln((d-1)\lambda_0) + \ln\left(\frac{d}{d-1}\right) \\
        &= \frac{1}{d} \ln\left( \frac{d^d}{(d-1)^{d+1} \lambda_0} \right) > 0,
    \end{align*}
    where we have used that the function $\psi(t) = -2 t + \ln(1 + t)$ is strictly decreasing when $t > 0$. 
    Then combining with Claim \ref{claim:hard-core:H}, we get the desired result. 
    
    \begin{remark}
        Here we provide some explanations on how to take $x_0$ as Equation (\ref{def:hard-core:x0}). 
        View $s$ as a function with respect to $x_0$, that is $s(x_0)$ is the solution to the Equation (\ref{claim:hard-core:s}). We want there exists $x_0$ such that
        \begin{align*}
            F(x_0) \triangleq G(s(x_0)) = x_0 - 2 \lambda e^{-d s(x_0)} + \ln\left(1 + \lambda e^{-d s(x_0)}\right) > 0. 
        \end{align*}
        
        By the definition of $s(x_0)$, we have
        \begin{align*}
            d(s'(x_0) + 1) &= - 2 \lambda d e^{-d s(x_0)} s'(x_0), \\
            s'(x_0) &= -\frac{1}{1 + 2 \lambda e^{-d s(x_0)}}.
        \end{align*}
        Hence $s(x_0)$ is strictly decreasing. 
        Next, note that 
        \begin{align*}
            F'(x_0) &= 1 + 2 \lambda d e^{-d s(x_0)} s'(x_0) - \frac{\lambda d e^{-d s(x_0)}}{1 + \lambda e^{-d s(x_0)}} s'(x_0) \\
            &= \frac{1 - (d - 1) \lambda e^{-d s(x_0)}}{1 + \lambda e^{-d s(x_0)}},
        \end{align*}
        which implies that $F(x_0)$ achieves its maximum value when $\lambda e^{-d s(x_0)} = \frac{1}{d-1}$ by $\psi(x_0) = \lambda e^{-d s(x_0)}$ is strictly increasing. 
        
        Letting $\lambda e^{-d s(x_0)} = \frac{1}{d-1}$, we have $s(x_0) = \frac{1}{d} \ln((d-1) \lambda)$. Then by the definition of $s(x_0)$, there holds
        \begin{align*}
            x_0 &= \frac{2}{d} (1 + \lambda e^{-d s(x_0)}) - s(x_0) \\
            &= \frac{2}{d-1} - \frac{1}{d} \ln((d-1) \lambda).
        \end{align*}
        And it is clear that
        \begin{align*}
            F(x_0) &= x_0 - \frac{2}{d - 1} + \ln\left(\frac{d}{d-1}\right) \\
            &= \frac{1}{d} \ln\left(\frac{d^d}{(d-1)^{d+1}\lambda} \right) > 0.
        \end{align*}
    \end{remark}
    
    \textbf{(2) The case $\lambda_0 < 0$. }
    
    At first, we suppose that $k < k_0 \triangleq \frac{\pi}{2 d (x_0 - x_1)}$ and $\lambda \in [\lambda_0, 0)$. 
    
    With setting 
    \begin{align}\label{def:hard-core:x0:1}
        x_0 = \frac{1}{d+1} \ln\left( \frac{1}{d |\lambda_0|} \right),
    \end{align}
    we have
    \begin{align}
        1 + \lambda e^{d x_0} > e^{-x_0},
    \end{align}
    which is according to 
    \begin{align*}
        e^{x_0} = \left(\frac{1}{d |\lambda_0|}\right)^{\frac{1}{d+1}} 
        > \frac{d + 1}{d} \ge 1 + \frac{1}{d} \left\vert\frac{\lambda}{\lambda_0}\right\vert 
        = 1 - \lambda e^{d x_0},
    \end{align*}
    where we have recalled that $|\lambda_0| < \frac{d^d}{(d+1)^{d+1}}$.
    
    Then for $z = -x + i y \in U(x_0, x_1, k)$ with $x \in [-x_0, -x_1]$ and $y \in [0, k(x_0 + x)]$, we can conclude that 
    \begin{align*}
        1 + \re(\lambda e^{d z}) = 1 + \lambda e^{-d x} \cos(d y) 
        \ge 1 + \lambda e^{-d x} \ge 1 + \lambda e^{d x_0} > e^{-x_0} > 0.
    \end{align*}
    Define
    \begin{align*}
        r(x, y) &\triangleq \re(g_{\lambda, d}(z)) = -\frac{1}{2} \ln\left( 1 + \lambda^2 e^{-2 d x} + 2 \lambda e^{-d x} \cos(d y) \right), \\
        h(x, y) &\triangleq |\im(g_{\lambda, d}(z))| = \arctan\left( \frac{|\lambda| e^{-d x} \sin(d y)}{1 + \lambda e^{-d x} \cos(d y)} \right).
    \end{align*}
    Note that $d k y < \frac{\pi}{2}$, we have
    \begin{align*}
        r(x, y) \le - \frac{1}{2} \ln(1 + \lambda^2 e^{-2 d x} + 2 \lambda e^{-d x}) \le - \ln(1 + \lambda e^{d x_0}) < x_0,
    \end{align*}
    and
    \begin{align*}
        r(x, y) \ge -\frac{1}{2} \ln\left( 1 + \lambda^2 e^{-2 d x} \right) \ge - \frac{1}{2} \ln\left( 1 + \lambda_0^2 e^{2 d x_0} \right).
    \end{align*}
    Hence, to ensure $r(x, y) \in (x_1, x_0)$, it is enough to set 
    \begin{align}
        x_1 = - \frac{1}{2} \ln\left( 1 + \lambda_0^2 e^{2 d x_0} \right) - 1.
    \end{align} 
    
    Similar to the proof in the case $\lambda_0 > 0$, we just need to determine $x_0, k$ such that
    \begin{align*}
        J(x, y, k) &\triangleq k(x - r(x, y)) - h(x, y) > 0.
    \end{align*}
    Note that
    \begin{align*}
        \frac{\partial J(x, y, k)}{\partial y} = -\frac{ d \lambda e^{-dx} (\lambda e^{-dx} + \cos(d y) - k \sin(d y))}{1 + \lambda^2 e^{-2dx} + 2 \lambda e^{-dx} \cos(d y))}.
    \end{align*}
    
    Now suppose that 
    $
        k < \min\{1, \frac{\pi}{4 d (x_0 - x_1)}\},
    $
    then we have
    \begin{align*}
        \lambda e^{-d x} + \cos(d k (x_0 + x)) - k \sin(d k (x_0 + x)) > \cos(\pi/4) - k \sin(\pi/4) > 0,
    \end{align*}
    and consequently, $\frac{\partial J(x, y, k)}{\partial y} < 0$. 
    
    Again, we just need to ensure that
    \begin{align*}
        G(x) &\triangleq \frac{\partial J(x, k(x_0 + x), k)}{\partial k} \bigg\vert_{k = 0} \\
        &= x_0 + \frac{d(x + x_0) \lambda e^{-d x}}{1 + \lambda e^{-d x}} +  \ln\left( 1 + \lambda e^{- d x} \right) > 0.
    \end{align*}
    Just note that
    \begin{align*}
        G'(x) = -\frac{d^2 (x + x_0) \lambda e^{-d x}}{(1 + \lambda e^{-d x})^2} > 0,
    \end{align*}
    and 
    \begin{align*}
        G(x) \ge G(-x_0) = x_0 + \ln(1 + \lambda e^{-d x_0}) > 0.
    \end{align*}
    
    \begin{remark}
        Here we provide some explanations on how to take $x_0$ as Equation (\ref{def:hard-core:x0:1}). 
        
        In fact, $g_{\lambda, d}(x_0) \in U(x_0, x_1, k)$ is equivalent to
        \begin{align*}
            -\ln(1 + \lambda e^{d x_0}) &< x_0, ~~~\text{i.e.,} \\
            1 + \lambda e^{d x_0} &> e^{-x_0}.
        \end{align*}
        Hence, we need to ensure the 
        \begin{align*}
            1 + \lambda_0 e^{d x_0} - e^{-x_0} > 0
        \end{align*}
        Next, observe that the function $\psi(x) = 1 + \lambda_0 e^{d x} - e^{-x}$ achieves maximal value at point $x = \frac{1}{d+1} \ln\left( \frac{1}{d |\lambda_0|} \right)$ which is the reason we set $x_0$ in Equation (\ref{def:hard-core:x0:1}).
        
    \end{remark}
\end{proof}


\begin{lemma}\label{lem:hard-core:complex}
    For $x_0, x_1, k$ satisfies the condition in Lemma \ref{lem:hard-core:real}, there exists $\delta > 0$ such that for all $\lambda \in \gU([0, \lambda_0], \delta)$ there holds
    \begin{align*}
        \overline{g_{\lambda, \Delta-1}(U(x_0, x_1, k))} \subseteq U(x_0, x_1, k).
    \end{align*}
\end{lemma}

\begin{proof}
    Denote $\tilde{U} = U(x_0, x_1, k)$ and $d = \Delta -1$.
    For $\lambda \in [0, \lambda_0]$, by $\tilde{U}$ is a bounded open set and $\overline{g_{\lambda, d}(\tilde{U})} \subseteq \tilde{U}$, there exists $\eps > 0$ such that
    \begin{align*}
        \mathrm{dist}(\overline{g_{\lambda, d}(\tilde{U})}, \partial \tilde{U}) > \eps.
    \end{align*}
    
    Then based continuity of $g_{\lambda, d}$ with respect to $\lambda$ and compactness of $\overline{\tilde{U}}$, there exists $\delta_{\lambda}$ such that 
    \begin{align*}
        |g_{\hat{\lambda}, d}(z) - g_{\lambda, d}(z)| < \eps, ~~~\text{ for } \forall \hat{\lambda} \in \gU(\lambda, \delta_{\lambda}), \forall z \in \overline{\tilde{U}},
    \end{align*}
    % \begin{align*}
    %     \mathrm{dist}(w, \overline{g_{\lambda, d}(\tilde{U})}) < \eps/2 
    %     ~~~\text{ for } \forall \hat{\lambda} \in \gU(\lambda, \delta_{\lambda}), \forall w \in \overline{g_{\hat{\lambda}, d}(\tilde{U})},
    % \end{align*}
    which implies that 
    \begin{align*}
        g_{\hat\lambda, d}(\tilde{U}) \subseteq \tilde{U}
        ~~~\text{ for } \forall \hat{\lambda} \in \gU(\lambda, \delta_{\lambda}).
    \end{align*}
    
    Next, observe that $[0, \lambda_0] \subseteq \bigcup_{\lambda \in [0, \lambda_0]} \gU(\lambda, \delta_{\lambda})$, then there exists $\lambda_1, \dots, \lambda_n$ such that
    \begin{align*}
        [0, \lambda_0] \subseteq \bigcup_{i=1}^n \gU(\lambda_i, \delta_{\lambda_i}).
    \end{align*}
    It is clearly that there exists $\delta$ such that
    \begin{align*}
        \gU([0, \lambda_0], \delta) \subseteq \bigcup_{i=1}^n \gU(\lambda_i, \delta_{\lambda_i}),
    \end{align*}
    which completes our proof.
\end{proof}

